Dynamic Complementarity Conditions and Whole-Body Trajectory Optimization for Humanoid Robot Locomotion

The paper presents a planner to generate walking trajectories by using the centroidal dynamics and the full kinematics of a humanoid robot. The interaction between the robot and the walking surface is modeled explicitly via new conditions, the \emph{Dynamical Complementarity Constraints}. The approach does not require a predefined contact sequence and generates the footsteps automatically. We characterize the robot control objective via a set of tasks, and we address it by solving an optimal control problem. We show that it is possible to achieve walking motions automatically by specifying a minimal set of references, such as a constant desired center of mass velocity and a reference point on the ground. Furthermore, we analyze how the contact modelling choices affect the computational time. We validate the approach by generating and testing walking trajectories for the humanoid robot iCub.

==> tex/ConstraintsJacobian.tex <==
\section{Jacobians of Kinematic and Dynamic Quantities}\label{chap:jacobians}

In this appendix, we present the partial derivatives of several quantities exploited in Sec. \ref{sec:oc}. 
As discussed in Sec. \ref{chap:experiments}, the optimal control problem is turned into an optimization problem and solved through off-the-shelf solvers. Such tools need to evaluate the partial derivatives of cost and constraint functions. To this end, we define an expression for those derivatives which are not trivially computable, usually involving non-linear functions of the variables considered in Eq. \eqref{eq:dp_state_control}, namely in $\bm{\mathcal{X}}$ and $\bm{\mathcal{U}}$. The dissertation shown here complements the results of \cite{carpentier2018analytical}\modtext{, adding the analytical partial derivatives of quantities like the centroidal momentum}.

\subsection{Partial derivative of a rotated vector} \label{sec:rotationPartialDer}
In this section, we face the partial derivatives computation of expressions involving a rotation matrix. A possible example is given by Eq. \eqref{eq:quaternionLeftDer}, where we seek to find the partial derivative of ${}^\mathcal{I}\bm{R}_B {}^B\bm{v}_{\mathcal{I},B}$ with respect to the base quaternion $^{\mathcal{I}} \bm{\rho}_B$. The computation of  $\frac{\partial}{\partial ^{\mathcal{I}} \bm{\rho}_B} {}^\mathcal{I}\bm{R}_B$ would result in a tensor, difficult to be handled. Indeed, it is easier to consider the case where the rotation matrix is multiplied by a generic vector $\bm{\chi} \in \mathbb{R}^3$.

Define $\bm{R} \in SO(3)$ as a generic rotation matrix and $\bm{\rho} \in \mathbb{H}$ the corresponding quaternion. We can rewrite the product $\bm{R} \bm{\chi}$ by using the Rodrigues formula \cite{murray2017mathematical}:
\begin{equation} \label{eq:rodriguesFormula}
\bm{R} \bm{\chi} = \bm{\chi} + 2\rho_w \bm{r}^\wedge \bm{\chi} + 2\bm{r}^\wedge \bm{r}^\wedge\bm{\chi},
\end{equation}
where
\begin{equation}
\bm{r} = \begin{bmatrix}
\rho_i \\
\rho_j \\
\rho_k
\end{bmatrix}
\end{equation}
contains the imaginary part of the quaternion and $\rho_w$ is its real part.
Thus:
\begin{IEEEeqnarray}{RCL}
	\IEEEyesnumber \phantomsection
\frac{\partial}{\partial \rho_w} \bm{R} \bm{\chi} &=& 2\bm{r}^\wedge\bm{\chi}, \nonumber\\
\frac{\partial}{\partial \bm{r}} \bm{R} \bm{\chi} &=& -2\rho_w \bm{\chi}^\wedge + 2 \frac{\partial}{\partial \bm{r}}\left(\bm{r}^\wedge\right) \bm{r}^\wedge \bm{\chi} + 2 \bm{r}^\wedge \frac{\partial}{\partial \bm{r}}\left(\bm{r}^\wedge\right)\bm{\chi}, \nonumber\\
&=& -2\rho_w\bm{\chi}^\wedge - 2 \left(\bm{r}^\wedge \bm{\chi }\right)^\wedge - 2 \bm{r}^\wedge
\bm{\chi}^\wedge, \nonumber \\
\frac{\partial}{\partial \bm{\rho}} \bm{R} \bm{\chi} &=& \begin{bmatrix}
 2\bm{r}^\wedge\bm{\chi} & -2\rho_w\bm{\chi}^\wedge - 2 \left(\bm{r}^\wedge \bm{\chi }\right)^\wedge - 2 \bm{r}^\wedge
 \bm{\chi}^\wedge
\end{bmatrix}. \IEEEyesnumber \label{eq:rotationDerivative}
\end{IEEEeqnarray}
Here we extensively used the property $(\bm{x})^\wedge \bm{y} = -(\bm{y})^\wedge \bm{x}$.

\subsection{Partial derivatives of a non unitary quaternion}\label{sec:normalizedQuaternion}
The quaternion modulus constraint can be broken across solver iterations. In fact, a generic solver can search over an unfeasible region while reaching the optimal solution. When computing the partial derivatives involving the base quaternion, we are implicitly assuming that it expresses a rotation (see for example Eq. \eqref{eq:rodriguesFormula}). This is true only if it has unit modulus. In order to satisfy this assumption, we have to normalize the quaternion before using it:
\begin{equation}
\bm{\rho}^N = \frac{\bm{\rho}}{\|\bm{\rho}\|} = \frac{\bm{\rho}}{\sqrt{\bm{\rho}^\top\bm{\rho}}}.
\end{equation}
This means that in order to compute the partial derivatives with respect to the not unitary quaternion, we have to perform the following operations:
\begin{equation}
\frac{\partial (\cdot)}{\partial \bm{\rho}} = \frac{\partial (\cdot)}{\partial \bm{\rho}^N} \frac{\partial \bm{\rho}^N}{\partial \bm{\rho}}.
\end{equation}
The first component, $\frac{\partial (\cdot)}{\partial \bm{\rho}^N}$, is the partial derivative of a generic function considering a normalized quaternion. For what concerns the second part instead:
\begin{IEEEeqnarray}{RCL}
	\phantomsection \IEEEyesnumber \label{eq:normalizedQuaternonDerivative}
	\frac{\partial \bm{\rho}^N}{\partial \bm{\rho}} &=& \frac{1}{\|\bm{\rho}\|}\bm{I}_4 - \left(\bm{\rho}^\top\bm{\rho}\right)^{-\frac{3}{2}}\bm{\rho} \bm{\rho}^\top, \IEEEyessubnumber \\
	&=& \frac{1}{\left(\bm{\rho}^\top\bm{\rho}\right)\|\bm{\rho}\|}\left(\left(\bm{\rho}^\top\bm{\rho}\right)\bm{I}_4 - \bm{\rho}\bm{\rho}^\top\right). \IEEEyessubnumber \label{eq:quaternionCorrection}
\end{IEEEeqnarray}
Thus, Eq. \eqref{eq:quaternionCorrection} must be multiplied on the right of all derivatives that consider an unit quaternion.

\subsection{Partial derivatives of adjoint matrices}\label{sec:adjoint_derivatives}
In this section, we present the partial derivative of an adjoint transform with respect to joint values. Let us consider two frames $P$ and $C$ connected through a single joint $j$. The time derivative of the adjoint matrix ${}^P\bm{X}_C$ is
\cite[Eq. (2.36)]{traversaro2017thesis}:
\begin{equation}
{}^P\dot{\bm{X}}_C = {}^P\bm{X}_C \left({}^C\bm{V}_{P,C}\times \right).
\end{equation}
The operator $\times$ is defined such that, given a vector ${}^C\textbf{s}_{P,C} = \left[{}^C \bm{v}_{P,C}^\top {}^C \bm{\omega}_{P,C}^\top\right]^\top$ we obtain:
\begin{equation}
{}^C\textbf{s}_{P,C}\times := 
\begin{bmatrix}
{}^C \bm{\omega}^\wedge_{P,C} & {}^C \bm{v}^\wedge_{P,C} \\
0_{3\times3} & {}^C \bm{\omega}^\wedge_{P,C}
\end{bmatrix}.
\end{equation}
From \cite[Lemma (3.5)]{traversaro2017thesis} we have
\begin{equation}
{}^C\textbf{V}_{P,C} = {}^C\textbf{s}_{P,C} ~\dot{s}_j,
\end{equation}
thus we finally obtain
\begin{equation}\label{eq:adjoint_partial_derivative}
\frac{\partial}{\partial s_j} {}^P\bm{X}_C = {}^P\bm{X}_C \left({}^C\textbf{s}_{P,C}\times \right).
\end{equation}

Let us consider now a more generic case where ${}^D\bm{X}_E$ defines a transformation between two frames, $D$ and $E$, rigidly attached to the robot. The partial derivative with respect to $s_j$ depends on whether joint $j$ belongs to the kinematic tree connecting $D$ to $E$, here defined as $\pi_D(E)$. If this is the case:
\begin{equation}
	{}^D\bm{X}_E = {}^D\bm{X}_P {}^P\bm{X}_C {}^C\bm{X}_E,
\end{equation}	
where only the transformation ${}^P\bm{X}_C$ depends on $s_j$. As a consequence
\begin{equation}\label{eq:multiple_adjoints_derivative}
	\begin{split}
		\frac{\partial}{\partial s_j} {}^D\bm{X}_E &=  {}^D\bm{X}_P {}^P\bm{X}_C \left({}^C\textbf{s}_{P,C}\times \right){}^C\bm{X}_E, \\
		&= {}^D\bm{X}_C \left({}^C\textbf{s}_{P,C}\times \right){}^C\bm{X}_E.
	\end{split}
\end{equation}
If instead $j \notin \pi_D(E)$ the partial derivative is null. To summarize
\begin{equation}\label{eq:adjoint_derivative}
	\frac{\partial}{\partial s_j} {}^D\bm{X}_E = \begin{cases}
	{}^D\bm{X}_C \left({}^C\textbf{s}_{P,C}\times \right){}^C\bm{X}_E, &\text{if } j \in \pi_D(E),\\
	0 &\text{otherwise}.
	\end{cases} 
\end{equation}

Analogously, it is possible to define the partial derivative of the 6D force coordinate transformation ${}_P\bm{X}^C$.
In particular,
\begin{equation}\label{eq:adjoint_wrench_derivative}
\frac{\partial}{\partial s_j} \left({}_P \bm{X}^C\right) = {}_{P} \bm{X}^C {}^C\textbf{s}_{P,C}\bar{\times}^*.
\end{equation}
The operator $\bar{\times}^*$ is defined such that, given ${}^C\textbf{s}_{P,C} = \left[{}^C \bm{v}_{P,C}^\top {}^C \bm{\omega}_{P,C}^\top\right]^\top$ we obtain \cite[Eq. (2.50)]{traversaro2017thesis}:
\begin{equation}
{}^C\textbf{s}_{P,C}\bar{\times}^* := 
\begin{bmatrix}
{}^C \bm{\omega}^\wedge_{P,C} & \bm{0}_{3\times3}  \\
{}^C \bm{v}^\wedge_{P,C} & {}^C \bm{\omega}^\wedge_{P,C}
\end{bmatrix}.
\end{equation}

\subsection{Partial derivatives of transformation matrices}\label{sec:rel_transf_derivative}

The relative transform ${}^D\bm{H}_E$ determines a change of coordinate for a generic vector ${}^E\bm{\chi}$, such that:
\begin{equation}\label{eq:generic_transform}
	{}^D\bm{\chi} = {}^D\bm{H}_E {}^E\bm{\chi}.
\end{equation}
Assuming ${}^E\bm{\chi}$ to be constant, this equation would depend only on the joint values connecting the two frames. In order to compute the partial derivative with respect to a generic joint value $s_j$, first we can rewrite Eq. \eqref{eq:generic_transform} as 
\begin{equation}
	{}^D\bm{\chi} = {}^D\bm{R}_E {}^E\bm{\chi} + {}^D\bm{o}_E.
\end{equation}

\subsubsection{Relative position}
The partial derivative of a relative position with respect to joint values can be obtained through the relative Jacobian. Denoting ${}^E\bm{J}_{D,E}$ as the \emph{left-trivialized} Jacobian, the relative \emph{left-trivialized} velocity is equal to
\begin{equation}
	{}^E\bm{V}_{D,E} = \begin{bmatrix}
	{}^D\bm{R}_E^\top ~ {}^D\dot{\bm{o}}_E \\
	{}^E\bm{\omega}_{D,E}
	\end{bmatrix} = {}^E\bm{J}_{D,E} \dot{\bm{s}},
\end{equation}
from which we obtain 
\begin{equation}
	{}^D\dot{\bm{o}}_E = {}^D\bm{R}_E\begin{bmatrix}
	\mathds{1}_3 & \bm{0}_{3\times3}
	\end{bmatrix} {}^D\bm{J}_{D,E}~\dot{\bm{s}} = \frac{\partial {}^D\bm{o}_E}{\partial s} \frac{\partial s}{\partial t},
\end{equation}
hence
\begin{equation}
	\frac{\partial}{\partial \bm{s}} {}^D\bm{o}_E = {}^D\bm{R}_E\begin{bmatrix}
	\mathds{1}_3 & \bm{0}_{3\times3}
	\end{bmatrix} {}^D\bm{J}_{D,E}.
\end{equation}
Assuming $j \in \pi_D(E)$, the partial derivative w.r.t joint $j$ consists in
\begin{equation}
	\frac{\partial}{\partial s_j} {}^D\bm{o}_E = {}^D\bm{R}_E\begin{bmatrix}
	\mathds{1}_3 & \bm{0}_{3\times3}
	\end{bmatrix}{}^E \bm{X}_C {}^C\textbf{s}_{P,C}.
\end{equation}

\subsubsection{Relative rotation}
The partial derivative of ${}^D\bm{R}_E {}^E\bm{\chi}$ instead requires some manipulation. In particular it is possible to exploit the result of Eq. \eqref{eq:adjoint_derivative} exploiting the fact that the upper left block of the adjoint matrix contains the rotation between the two frames. Thus, we have
\begin{equation}
	{}^D\bm{R}_E {}^E\bm{\chi} = \begin{bmatrix}
	\mathds{1}_3 & \bm{0}_{3\times3}
	\end{bmatrix} {}^D\bm{X}_E \begin{bmatrix}
	{}^E\bm{\chi} \\
	\bm{0}_{3\times 1}
	\end{bmatrix},
\end{equation}
or alternatively
\begin{equation}
{}^D\bm{R}_E {}^E\bm{\chi} = \begin{bmatrix}
\mathds{1}_3 & \bm{0}_{3\times3}
\end{bmatrix} {}^D\bm{X}_E \begin{bmatrix}
\mathds{1}_3 \\ \bm{0}_{3\times3}
\end{bmatrix} {}^E\bm{\chi}.
\end{equation}
Assuming $j \in \pi_D(E)$, we obtain
\begin{equation*}
	\frac{\partial}{\partial s_j} {}^D\bm{R}_E{}^E\bm{\chi} = \begin{bmatrix}
	\mathds{1}_3 & \bm{0}_{3\times3}
	\end{bmatrix} {}^D\bm{X}_C \left({}^C\textbf{s}_{P,C}\times \right){}^C\bm{X}_E \begin{bmatrix}
	{}^E\bm{\chi} \\
	\bm{0}_{3\times 1}
	\end{bmatrix},
\end{equation*}
allowing us to build $\frac{\partial}{\partial \bm{s}} {}^D\bm{R}_E{}^E\bm{\chi}$ by column.

\subsubsection{Transformations relative to the inertial frame} \label{sec:base_transforms_derivative}
Eq. \eqref{eq:dp_point_consistency} presents a coordinate transformation of a (fixed) vector ${}^\text{foot}{}_i \bm{p}$. The transformation matrix ${}^\mathcal{I} \bm{H}_\text{foot}$ depends on the base pose and on all the joints connecting the foot frame to the base. It is possible to split this relation in the following two equations:
\begin{IEEEeqnarray}{RCL}
	\phantomsection \IEEEyesnumber
	{}_i \bm{p} &=& {}^\mathcal{I} \bm{H}_B {}^B{}_i \bm{p}, \IEEEyessubnumber \label{eq:transform_base_to_I}\\
	{}^B{}_i \bm{p} &=& {}^B \bm{H}_\text{foot} {}^\text{foot}{}_i \bm{p}. \IEEEyessubnumber \label{eq:transform_point_to_base}
\end{IEEEeqnarray}
Eq. \eqref{eq:transform_point_to_base} depends only on joint positions and its partial derivative can be computed as showed in Sec. \ref{sec:rel_transf_derivative}. On the other hand, Eq. \eqref{eq:transform_base_to_I} depends only on the base position ${}^\mathcal{I}\bm{p}_B$ and its orientation, expressed through the quaternion ${}^\mathcal{I}\bm{\rho}_B$. By rewriting it as
\begin{equation}
	{}_i \bm{p} = {}^\mathcal{I} \bm{R}_B {}^B{}_i \bm{p} + {}^\mathcal{I}\bm{p}_B,
\end{equation}
the derivative with respect to the base position can be computed trivially, while $\frac{\partial}{\partial {}^\mathcal{I}\bm{\rho}_B} \left({}^\mathcal{I} \bm{R}_B {}^B{}_i \bm{p}\right)$ can be computed as in Sec. \ref{sec:rotationPartialDer}.

% \subsection{Partial derivatives of the base velocity}
% The \emph{left-trivialized} base velocity is defined as 
% \begin{equation}
% 	{}^B\bm{V}_{\mathcal{I},B} = \begin{bmatrix}
% 	{}^B\bm{v}_{\mathcal{I},B} \\
% 	{}^B\bm{\omega}_{\mathcal{I},B}
% 	\end{bmatrix}.
% \end{equation}
% While the linear part is contained in the optimization variables, the angular part is not. In fact, the quaternion time derivative is used instead inside $\bm{\mathcal{U}}$. As shown in Eq. \eqref{eq:base_angular_velocity}, the base angular velocity depends linearly on the quaternion derivative, while the map $\bm{\mathcal{G}}$ depends on the base quaternion ${}^\mathcal{I}\bm{\rho}_B$. For simplicity, let us drop the superscripts and define $\bm{\omega}$ as the \emph{left-trivialized} angular velocity. $r$ is the imaginary part of the base quaternion and $\rho_w$ is its real part while $\dot{\bm{r}}$ and $\dot{\rho}_w$ compose the quaternion derivative. Then, from \cite[Sec. 1.5.4]{graf2008quaternions}, we have
% \begin{equation}
% 	\bm{\omega} = 2\left( \rho_w\dot{\bm{r}} - \dot{\rho}_w\bm{r} - \bm{r}^\wedge\dot{\bm{r}} \right).
% \end{equation}
% We finally obtain
% \begin{equation}
% 	\frac{\partial}{\partial \bm{\rho}}\bm{\omega} = \begin{bmatrix}
% 	\dot{\bm{r}} & \dot{\bm{r}}^\wedge - \rho_w \mathds{1}_3
% 	\end{bmatrix}.
% \end{equation}

\subsection{Partial derivatives of a link velocity}\label{sec:velocity_derivative}
Let us consider the \emph{left-trivialized} velocity of a generic link $L$.
This element depends on a series of quantities, namely:
\begin{itemize}
	\item joint positions $\bm{s}$,
	\item joint velocities $\dot{\bm{s}}$,
	\item base velocity ${}^B\bm{V}_{\mathcal{I},B}$.
\end{itemize}
The partial derivative with respect to $\dot{\bm{s}}$ and ${}^B\bm{V}_{\mathcal{I},B}$ are trivially obtained from the corresponding \emph{left-trivialized} Jacobian. Contrarily, the partial derivative with respect to joint values requires some manipulation.

At first, we compute the partial derivative of a velocity relative to the robot base (hence not depending on base quantities). Subsequently, the base velocity is added. 
%In Eq. \eqref{eq:velocity_expanded}, the matrix ${}^L\bm{X}_{m_B(k)}$ depends on (a subset of) the joint variables.
By considering one single joint at a time, the partial derivative of ${}^L\bm{V}_{B,L}$ is:
\begin{equation}
\begin{split}
&\frac{\partial}{\partial s_j} {}^L\bm{V}_{B,L} =\\
&\sum_{k \in \pi_B(L)} \left({}^L\bm{X}_C \left(\frac{\partial}{\partial s_j} {}^C\bm{X}_P \right)  {}^P\bm{X}_{m_B(k)}  {}^{m_B(k)}\textbf{s} \right) \dot{s}_k,
\end{split}
\end{equation}
where $C = m_B(j)$, i.e. the child of joint $j$ and $P = \lambda_B\left(j\right)$ its parent.
By applying Eq. \eqref{eq:adjoint_partial_derivative} we obtain:
\begin{equation*}
\begin{split}
&\frac{\partial}{\partial s_j} {}^L\bm{V}_{B,L} =\\
&\sum_{k \in \pi_B(L)} \left( {}^L\bm{X}_C \left({}^C\bm{X}_P {}^P\textbf{s}_{C,P} \times \right)  {}^P\bm{X}_{m_B(k)}  {}^{m_B(k)}\textbf{s} \right) \dot{s}_k.
\end{split}
\end{equation*}

Note that, compared to Eq. \eqref{eq:adjoint_partial_derivative}, the order of $P$ and $C$ is inverted. We can restore the previous order by noting that 
\begin{equation}
\begin{split}
	{}^P\textbf{s}_{P,C} &= -{}^P\textbf{s}_{C,P}, \\
	{}^C\textbf{s}_{P,C} &= {}^C \bm{X}_P {}^P\textbf{s}_{P,C}.
\end{split}
\end{equation}
In addition, it is possible to exploit the following property:
\begin{equation}
	\left( \left( {}^P\bm{X}_C{}^C\textbf{s}_{P,C} \right) \times\right) =  {}^P\bm{X}_C\left({}^C\textbf{s}_{P, C} \times\right) {}^C\bm{X}_P.
\end{equation}
so that
\begin{equation}
	{}^C\bm{X}_P {}^P\textbf{s}_{C,P} \times = -{}^C\textbf{s}_{P,C} \times {}^C\bm{X}_P.
\end{equation}
As a consequence, we obtain
\begin{IEEEeqnarray}{L}
	\IEEEyesnumber \phantomsection
	\frac{\partial}{\partial s_j} {}^L\bm{V}_{B,L} \nonumber \\
	= {-}\sum_{k \in \pi_B(L)} \left( {}^L\bm{X}_C \left({}^C\textbf{s}_{P,C} {\times} {}^C\bm{X}_P\right)  {}^P\bm{X}_{m_B(k)}  {}^{m_B(k)}\textbf{s} \right) \dot{s}_k, \nonumber \\
	= -\sum_{k \in \pi_B(L)} \left( {}^L\bm{X}_C {}^C\textbf{s}_{P,C} \times {}^C\bm{X}_{m_B(k)}  {}^{m_B(k)}\textbf{s} \right) \dot{s}_k. 
\end{IEEEeqnarray}
Joint $j$ must also belong to $\pi_B(L)$ and $k \leq j$, i.e. joint $j$ must be in the chain from $k$ to $L$ (using $B$ as base), otherwise the matrix ${}^L\bm{X}_{m_B(k)}$ does not depend on $s_j$. Henceforth, the summation is on the part of the kinematic tree which starts from $B$ and ends in $C$. This set corresponds to $\pi_B(C)$. Thus, we have:
\begin{equation*}
\frac{\partial}{\partial s_j} {}^L\bm{V}_{B,L} =  -{}^L\bm{X}_C {}^C\textbf{s}_{P,C} \times  \sum_{k \in \pi_B(C)} \left({}^C\bm{X}_{m_B(k)}  {}^{m_B(k)}\textbf{s} \right) \dot{s}_k.
\end{equation*}
Applying \cite[Lemma (3.5)]{traversaro2017thesis} to the summation on the right hand side, we can write  
\begin{equation}\label{eq:velocityPartialDerivativeCompact}
\frac{\partial}{\partial s_j} {}^L\bm{V}_{B,L} = -{}^L\bm{X}_C {}^C\textbf{s}_{P,C} \times {}^C \bm{V}_{B,C}.
\end{equation}
	
The velocity of link $L$ with respect to an inertial frame $\mathcal{I}$ is obtained as
\begin{equation}\label{eq:velocity_inertial}
{}^L\bm{V}_{\mathcal{I}, L} = {}^L\bm{X}_B{}^B\bm{V}_{\mathcal{I}, B} + {}^L\bm{V}_{B, L},
\end{equation}
hence, its partial derivative w.r.t. the position of joint $j$ is
\begin{equation}\label{eq:velocityExpansion}
\frac{\partial}{\partial s_j} {}^L\bm{V}_{\mathcal{I},L} = \frac{\partial}{\partial s_j}  {}^L\bm{X}_B {}^B\bm{V}_{\mathcal{I},B} + \frac{\partial}{\partial s_j} {}^L\bm{V}_{B,L}.
\end{equation}
The second part is obtained through Eq. \eqref{eq:velocityPartialDerivativeCompact}, while the first is computed as in Eq. \eqref{eq:adjoint_derivative} obtaining
\begin{equation}\label{eq:base_part_Velocity_derivative}
\begin{split}
&\frac{\partial}{\partial s_j}  {}^L\bm{X}_B {}^B\bm{V}_{\mathcal{I},B} = \\
& =\begin{cases}
-{}^L\bm{X}_C {}^C\textbf{s}_{P,C} \times {}^C\bm{X}_B {}^B\bm{V}_{\mathcal{I},B}, & j \in \pi_B(L), \\
0 & \text{otherwise}.
\end{cases}
\end{split}
\end{equation}
Finally, substituting Eq. \eqref{eq:velocityPartialDerivativeCompact} and Eq. \eqref{eq:base_part_Velocity_derivative} into Eq. \eqref{eq:velocityExpansion}, we obtain
\begin{equation}\label{eq:velocity_inertial_derivative}
\frac{\partial}{\partial s_j} {}^L\bm{V}_{\mathcal{I},L} = \begin{cases}
{}^L\bm{X}_C {}^C\textbf{s}_{P,C} \times \left(-{}^C\bm{V}_{A,C}\right), & j \in \pi_B(L) \\
0 & \text{otherwise}.
\end{cases}
\end{equation}

\subsection{Partial derivatives of the CoM position}\label{sec:com_jacobian}
Eq. \eqref{eq:comConsistency} imposes that $\bm{x}$ should match the CoM position computed from forward kinematics, $\text{CoM}({}^\mathcal{I}\bm{p}_B, {}\mathcal{I}\bm{\rho}_B, s)$.
%By definition, the center of mass (CoM) $\bm{x}$ corresponds to the weighted average of all the links CoM position:
%\begin{equation}\label{eq:com_definition}
%\bm{x} = {}^\mathcal{I} \bm{H}_B\sum_i \frac{m_i}{m}{}^{B} \bm{H}_i  ~ {}^i\textbf{p}_{\text{CoM}},
%\end{equation}
%where ${}^i\textbf{p}_{\text{CoM}} \in \mathbb{R}^3$ is the (constant) CoM position of link $i$ expressed in $i$ coordinates. $m, m_i \in \mathbb{R}$ are respectively the robot total mass and the $i$-th link mass. 
In order to compute the partial derivative of such function w.r.t base and joint variables, we can resort to the CoM jacobian $\bm{J}_\text{CoM}$. We can split $\bm{J}_\text{CoM}$ as follows:
\begin{equation}
\bm{J}_\text{CoM} = \begin{bmatrix}
\bm{J}_\text{CoM}^{v_b} & \bm{J}_\text{CoM}^{\omega_b} & \bm{J}_\text{CoM}^{\dot{s}}
\end{bmatrix},
\end{equation}
such that
\begin{equation}
	\bm{v}_\text{CoM} = \begin{bmatrix}
	\bm{J}_\text{CoM}^{v_b} & \bm{J}_\text{CoM}^{\omega_b} & \bm{J}_\text{CoM}^{\dot{s}}
	\end{bmatrix} \begin{bmatrix}
		{}^\mathcal{I}\dot{\bm{p}}_{B} \\
		{}^\mathcal{I}\bm{\omega}_{\mathcal{I},B} \\
		\dot{\bm{s}}
	\end{bmatrix}.
\end{equation}
where $\bm{v}_\text{CoM}$ is the CoM velocity relative to the inertial frame $\mathcal{I}$, expressed in a frame located on the CoM having orientation parallel to $\mathcal{I}$ (\emph{mixed} representation). Thanks to this choice of frame, the CoM jacobian $\bm{J}_\text{CoM}$ maps the base position time derivative ${}^\mathcal{I}\dot{\bm{p}}_{B}$, the \emph{right-trivialized} base angular velocity ${}^\mathcal{I}\bm{\omega}_{\mathcal{I},B}$ and the joint time derivative into the CoM velocity. Thus, we have:
\begin{IEEEeqnarray}{RCL}
	\frac{\partial}{\partial s} \text{CoM}({}^\mathcal{I}\bm{p}_B, {}\mathcal{I}\bm{\rho}_B, s) &=& \bm{J}_\text{CoM}^{\dot{s}}, \\
	\frac{\partial}{\partial {}^\mathcal{I}\bm{p}_B} \text{CoM}({}^\mathcal{I}\bm{p}_B, {}\mathcal{I}\bm{\rho}_B, s) &=& \bm{J}_\text{CoM}^{v_b}.
\end{IEEEeqnarray}
For what concerns the rotation part, we need the partial derivative with respect to the quaternion. Given that we are considering a Jacobian in mixed representation, we need to map a quaternion derivative into an angular velocity expressed in an inertial frame (\emph{right-trivialized}). This relation is defined in \cite[Sec. 1.5.3]{graf2008quaternions}:
\begin{equation}\label{eq:quaternionMap}
{}^\mathcal{I}\bm{\omega}_{\mathcal{I},B} = 2\bm{E}~{}^\mathcal{I}\dot{\bm{\rho}}_B.
\end{equation}
Finally we have
\begin{equation} \label{eq:comJacQuaternion}
\frac{\partial}{\partial {}^\mathcal{I}\bm{\rho}_B} \text{CoM}({}^\mathcal{I}\bm{p}_B, {}\mathcal{I}\bm{\rho}_B, s) = 2\bm{J}_\text{CoM}^{\omega_b}\bm{E}.
\end{equation}

Alternatively, we can obtain these partial derivative by starting from the following relation:
\begin{equation}
	\bm{x} = {}^\mathcal{I} \bm{H}_B {}^B\bm{p}_\text{CoM},
\end{equation}
where ${}^B\bm{p}_\text{CoM} \in \mathbb{R}^3$ is the CoM position expressed in base coordinates. In this way, the partial derivatives w.r.t base position and quaternion can be computed as in Sec. \ref{sec:base_transforms_derivative} and we are left with the computation of $\frac{\partial}{\partial \bm{s}} {}^B \bm{p}_\text{CoM}$. Exploiting the results of Sec. \ref{sec:rel_transf_derivative} and the CoM definition of Eq. \eqref{eq:com_definition}, the partial derivative w.r.t. joint $j$ is the following
\begin{equation}\label{eq:base_com_derivative}
	\begin{split}
			&\frac{\partial}{\partial s_j} {}^B \bm{p}_\text{CoM} = \sum_{i : j \in \pi_B(i)} \frac{m_i}{m}\left({}^B\bm{R}_i\begin{bmatrix}
				\mathds{1}_3 & \bm{0}_{3\times3}
			\end{bmatrix}{}^i \bm{X}_C {}^C\textbf{s}_{P,C} + \right. \\
			&+\left. \begin{bmatrix}
				\mathds{1}_3 & \bm{0}_{3\times3}
			\end{bmatrix} {}^B\bm{X}_C \left({}^C\textbf{s}_{P,C}\times \right){}^C\bm{X}_i \begin{bmatrix}
			{}^i\bm{\rho}_{\text{CoM}} \\
			\bm{0}_{3\times 1}
		\end{bmatrix}\right),
	\end{split}
\end{equation}
where the summation is over those joints having $j$ in their path to the base.

\subsection{Partial derivatives of centroidal momentum}

In this section, we analyze Eq. \eqref{constr:CMM}. The partial derivative w.r.t the (\emph{left-trivialized}) base velocity and joint velocities consist in selecting the corresponding columns of the Centroidal Momentum Matrix $\bm{J}_\text{CMM}$ \cite{orin08}. In the following, we examine the dependency from the joint positions and base pose.

\subsubsection{Partial derivative w.r.t. CoM position and base pose}\label{sec:momentum_derivative_com}
Equation \eqref{eq:momentumExpanded} depends upon the base pose and CoM position only through matrix ${}_{\bar{G}} \bm{X}^B$.
We can rewrite Eq. \eqref{eq:momentumExpanded} as:
\begin{equation} \label{eq:momentumInBase}
{}_{\bar{G}} \bm{h} = {}_{\bar{G}} \bm{X}^\mathcal{I} {}_{\mathcal{I}} \bm{X}^B {}_{B} \bm{h}
\end{equation}
where ${}_{B} \bm{h}$ is the centroidal momentum expressed in base coordinates. We can expand Eq. \eqref{eq:momentumInBase}:
\begin{equation}
{}_{\bar{G}} \bm{h} = 
\begin{bmatrix}
\mathds{1}_3 & 0 \\
-\bm{x}^\wedge & \mathds{1}_3
\end{bmatrix}
\begin{bmatrix}
{}^{\mathcal{I}} \bm{R}_B & 0 \\
{}^{\mathcal{I}} \bm{p}^\wedge_B {}^{\mathcal{I}} \bm{R}_B  & {}^{\mathcal{I}} \bm{R}_B
\end{bmatrix}
\begin{bmatrix}
{}_{B} \bm{h}^{v} \\
{}_{B} \bm{h}^{\omega}
\end{bmatrix},
\end{equation}
obtaining
\begin{equation}
{}_{\bar{G}} \bm{h} = 
\begin{bmatrix}
{}^{\mathcal{I}} \bm{R}_B & 0 \\
{}^{\mathcal{I}} \bm{p}^\wedge_B {}^{\mathcal{I}} \bm{R}_B -\bm{x}^\wedge{}^{\mathcal{I}} \bm{R}_B  & {}^{\mathcal{I}} \bm{R}_B
\end{bmatrix}
\begin{bmatrix}
{}_{B} \bm{h}^{v} \\
{}_{B} \bm{h}^{\omega}
\end{bmatrix}.
\end{equation}
By substituting $\bm{x} = {}^{\mathcal{I}} \bm{R}_B {}^B\bm{p}_{\text{CoM}} + {}^\mathcal{I}\bm{p}_B$, exploiting the additivity property of the $\wedge$ operator and the rotational invariance of cross products, we obtain:
\begin{equation}
	{}_{\bar{G}} \bm{h} = 
	\begin{bmatrix}
	{}^{\mathcal{I}} \bm{R}_B & 0 \\
	-{}^B\bm{p}_{\text{CoM}}^\wedge  & {}^{\mathcal{I}} \bm{R}_B
	\end{bmatrix}
	\begin{bmatrix}
	{}_{B} \bm{h}^{v} \\
	{}_{B} \bm{h}^{\omega}
	\end{bmatrix}.
\end{equation}
Hence the centroidal momentum ${}_{\bar{G}} \bm{h}$ does not depend on the base position:
\begin{equation}
	\frac{\partial}{\partial {}^\mathcal{I}\bm{p}_B} {}_{\bar{G}} \bm{h} = 0.
\end{equation}

In order to compute the derivative w.r.t. the CoM position and the base quaternion, we can express the linear and angular momentum separately:
\begin{IEEEeqnarray}{RCL}
	\IEEEyesnumber \phantomsection\label{eq:AXBDerivative}
	{}_{\bar{G}} \bm{h}^v &=& {}^{\mathcal{I}} \bm{R}_B {}_{B} \bm{h}^{v}, \IEEEyessubnumber \\
	{}_{\bar{G}} \bm{h}^\omega &=& -{}^B\bm{p}_{\text{CoM}}^\wedge {}_B\bm{h}^{v} + {}^{\mathcal{I}} \bm{R}_B {}_{B} \bm{h}^{\omega} \IEEEyessubnumber 
\end{IEEEeqnarray}
For what concerns the partial derivatives of the rotation matrix with respect to the base quaternion, we can use the results of Section \ref{sec:rotationPartialDer}. Regarding the CoM position, we have: 
\begin{equation}
	\frac{\partial}{\partial {}^B\bm{p}_{\text{CoM}}}{}_{\bar{G}} \bm{h} = \begin{bmatrix}0_{3\times 3} \\ {}_{B} \bm{h}^{v\wedge}  \end{bmatrix}.
\end{equation}
The partial derivative w.r.t $\bm{x}$, i.e. $\frac{\partial {}^B\bm{p}_{\text{CoM}}}{\partial \bm{x}}$ can be easily computed by composition. Otherwise, it is possible to exploit Eq.\eqref{eq:base_com_derivative} to compute directly the partial derivative w.r.t joint variables for this component.

\subsubsection{Partial derivative with respect to joint values} \label{sec:CMMjoints}
Let us consider now the partial derivative w.r.t joint values:
\begin{equation} \label{eq:momentumJointDerivative}
\frac{\partial}{\partial s_j} {}_{\bar{G}} \bm{h} =\frac{\partial}{\partial s_j}\left({}_{\bar{G}} \bm{X}^B\right){}_{B} \bm{h} + {}_{\bar{G}} \bm{X}^B \frac{\partial}{\partial s_j} \left({}_{B} \bm{h} \right).
\end{equation}
The first derivative can be computed from the results of Sec. \ref{sec:momentum_derivative_com}. In this section we focus on $\frac{\partial}{\partial s_j} \left({}_{B} \bm{h} \right)$. 

The centroidal momentum expressed in base coordinates is the sum of all the link momenta expressed in the same frame. Hence:
\begin{equation}\label{eq:momentum_initial_derivative}
\frac{\partial}{\partial s_j} {}_{B} \bm{h} = \sum_i \frac{\partial}{\partial s_j} \left({}_{B} \bm{X}^i \right)  \bm{I}_i {}^i \bm{V}_{\mathcal{I},i} + \sum_i {}_{B} \bm{X}^i \bm{I}_i \frac{\partial}{\partial s_j}\left( {}^i \bm{V}_{\mathcal{I},i} \right).
\end{equation}
The derivative $\frac{\partial}{\partial s_j} \left({}_{B} \bm{X}^i \right)$ is obtained as in Eq. \eqref{eq:adjoint_wrench_derivative}, while Eq. \eqref{eq:velocity_inertial_derivative} presents the partial derivative of the link velocity. Thus, we can rewrite Eq. \eqref{eq:momentum_initial_derivative} as follows:
\begin{IEEEeqnarray}{RCL}
	\IEEEyesnumber \phantomsection
	\frac{\partial}{\partial s_j} {}_{B} \bm{h} &=& \sum_{i : j \in \pi_B(i)} \left( {}_{B} \bm{X}^C {}^C\textbf{s}_{P,C}\bar{\times}^* {}_C \bm{X}^i  \bm{I}_i {}^i \bm{V}_{\mathcal{I},i} +\right. \nonumber\\
	&&\left.- {}_{B} \bm{X}^i \bm{I}_i {}^i\bm{X}_C {}^C\textbf{s}_{P,C} \times \left({}^C\bm{V}_{\mathcal{I},C}\right) \right) \nonumber \\
	&=& {}_{B} \bm{X}^C {}^C\textbf{s}_{P,C}\bar{\times}^*  \left(\sum_{i : j \in \pi_B(i)} {}_C \bm{X}^i  \bm{I}_i {}^i \bm{V}_{\mathcal{I},i}\right) + \nonumber \\
	&&- \left(\sum_{i : j \in \pi_B(i)} {}_{B} \bm{X}^i \bm{I}_i {}^i\bm{X}_C\right) {}^C\textbf{s}_{P,C} \times \left({}^C\bm{V}_{\mathcal{I},C}\right), \nonumber
\end{IEEEeqnarray}
with $j$ connecting the child link $C$ to its parent $P$ and the sums being on the links which have $j$ in their path to the base.

\subsubsection{Partial derivative w.r.t base and joint velocities}
Eq. \eqref{eq:momentumExpanded} depends upon the base velocity ${}^B\bm{V}_{\mathcal{I},B}$ through ${}^i\bm{V}_{\mathcal{I},i}$. By using Eq. \eqref{eq:velocity_inertial}, we can write:
\begin{equation}
	\frac{\partial}{\partial {}^B\bm{V}_{\mathcal{I},B}} {}^i\bm{V}_{\mathcal{I},i} = {}^i\bm{X}_B,
\end{equation}
hence
\begin{equation}
	\frac{\partial}{\partial {}^B\bm{V}_{\mathcal{I},B}} {}_{\bar{G}} \bm{h} = {}_{\bar{G}} \bm{X}^B \sum_i {}_{B} \bm{X}^i \bm{I}_i {}^i\bm{X}_B.
\end{equation}
This corresponds to the first $6$ columns of the CMM matrix. The other rows corresponds to the partial derivative with respect to joint velocities. Given a generic joint $j$, the partial derivative w.r.t. $\dot{s}_j$ is:
\begin{equation}
	\frac{\partial}{\partial \dot{s}_j} {}_{\bar{G}} \bm{h} = {}_{\bar{G}} \bm{X}^B \sum_{i : j \in \pi_B(i)} {}_{B} \bm{X}^i \bm{I}_i {}^i\bm{X}_{C}  {}^{C}\textbf{s}_{P,C}.
\end{equation}
%where we used the relation presented in Eq. \eqref{eq:velocity_expanded}.


% \subsection{Partial derivatives of a quaternion as rotation error}

% Sec. \ref{sec:orientation_task} adopts a task which minimizes the rotation error of a generic frame attached to the robot. Since the reference orientation is expressed in the inertial frame $\mathcal{I}$, this error depends on the kinematic status of the robot, viz. joint positions and base pose.
% To compute the partial derivatives of the function $\texttt{quat}({}^A\tilde{\bm{R}}_\text{frame})$, let us start by considering the time derivative of the quaternion error $\bm{\rho}_{\text{err}}$ as in \cite[Section 1.5.4]{graf2008quaternions}:
% \begin{equation}
% \dot{\bm{\rho}}_\text{err} = \frac{1}{2} \bm{\mathcal{G}}(\bm{\rho}_{\text{err}})^\top \bm{\omega}_\text{err},
% \end{equation}
% where $\bm{\omega}_\text{err}$ is the \emph{left-trivialized} angular velocity. $\bm{\rho}_\text{err}$ is the quaternion associated to the rotation error matrix ${}^\mathcal{I}\tilde{\bm{R}}_\text{frame}={}^\mathcal{I}\bm{R}^{*\top}_\text{frame}{}^\mathcal{I}\bm{R}_\text{frame}$, while the \emph{left-trivialized} velocity $\bm{\omega}_\text{err}$ is obtained as:
% \begin{equation}
% \bm{\omega}_\text{err} = \left({}^\mathcal{I}\tilde{\bm{R}}_\text{frame}^\top{}^\mathcal{I}\dot{\tilde{\bm{R}}}_\text{frame}\right)^\vee.
% \end{equation}
% By substituting we have
% \begin{IEEEeqnarray}{RCL}
% 	\IEEEyesnumber \phantomsection
% 	\dot{\bm{\rho}}_\text{err} &=& \frac{1}{2} \bm{\mathcal{G}}(\bm{\rho}_{\text{err}})^\top\left({}^\mathcal{I}\tilde{\bm{R}}_\text{frame}^\top{}^\mathcal{I}\dot{\tilde{\bm{R}}}_\text{frame}\right)^\vee,  \nonumber\\
% 	&=& \frac{1}{2} \bm{\mathcal{G}}(\bm{\rho}_{\text{err}})^\top\left({}^\mathcal{I}\bm{R}^\top_\text{frame} {}^\mathcal{I}\bm{R}^{*}_\text{frame} \frac{\dif}{\dif t}\left({}^\mathcal{I}\bm{R}^{*\top}_\text{frame}{}^\mathcal{I}\bm{R}_\text{frame}\right)\right)^\vee,  \nonumber\\
% 	&=& \frac{1}{2} \bm{\mathcal{G}}(\bm{\rho}_{\text{err}})^\top\left({}^\mathcal{I}\bm{R}^\top_\text{frame} {}^\mathcal{I}\bm{R}^{*}_\text{frame} {}^\mathcal{I}\bm{R}^{*\top}_\text{frame}\frac{\dif}{\dif t}\left({}^\mathcal{I}\bm{R}_\text{frame}\right)\right)^\vee, \nonumber \\
% 	&=& \frac{1}{2} \bm{\mathcal{G}}(\bm{\rho}_{\text{err}})^\top\left({}^\mathcal{I}\bm{R}^\top_\text{frame}{}^\mathcal{I}\dot{\bm{R}}_\text{frame}\right)^\vee, \nonumber \\
% 	&=& \frac{1}{2} \bm{\mathcal{G}}(\bm{\rho}_{\text{err}})^\top {}^\text{frame}\bm{\omega}_{\mathcal{I}, \text{frame}},
% \end{IEEEeqnarray}
% with ${}^\text{frame}\bm{\omega}_{\mathcal{I}, \text{frame}}$ the \emph{left-trivialized} frame angular velocity. This velocity can be computed using the bottom three rows of the corresponding \emph{left-trivialized} Jacobian ${}^\omega \bm{J}$, where we drop the subscripts for the sake of simplicity:
% \begin{equation*}
% \begin{split}
% 	{}^\text{frame}\bm{\omega}_{\mathcal{I}, \text{frame}} &= {}^\omega \bm{J} \begin{bmatrix}
% 	{}^\mathcal{I}\dot{\bm{p}}_{B} \\
% 	{}^B\bm{\omega}_{\mathcal{I},B} \\
% 	\dot{\bm{s}}
% 	\end{bmatrix},\\
% 	&= \begin{bmatrix}
% 	{}^\omega \bm{J}^{v_b} & {}^\omega \bm{J}^{\omega_b} & {}^\omega \bm{J}^{\dot{s}}
% 	\end{bmatrix} \begin{bmatrix}
% 	{}^\mathcal{I}\dot{\bm{p}}_{B} \\
% 	2\bm{\mathcal{G}}({}^\mathcal{I}\bm{\rho}_{B}){}^\mathcal{I}\dot{\bm{\rho}}_B \\
% 	\dot{\bm{s}}
% 	\end{bmatrix}.
% \end{split}
% \end{equation*}
% Henceforth, the following derivatives are easily obtained:
% \begin{IEEEeqnarray}{RCL}
% 	\frac{\partial}{\partial {}^\mathcal{I}\bm{p}_{B}} \bm{\rho}_\text{err} &=& \frac{1}{2} \bm{\mathcal{G}}(\bm{\rho}_{\text{err}})^\top {}^\omega \bm{J}^{v_b}, \\
% 	\frac{\partial}{\partial {}^\mathcal{I}\bm{\rho}_{B}} \bm{\rho}_\text{err} &=& \bm{\mathcal{G}}(\bm{\rho}_{\text{err}})^\top {}^\omega \bm{J}^{\omega_b}\bm{\mathcal{G}}({}^\mathcal{I}\bm{\rho}_{B}), \\
% 	\frac{\partial}{\partial \bm{s}} \bm{\rho}_\text{err} &=& \frac{1}{2} \bm{\mathcal{G}}(\bm{\rho}_{\text{err}})^\top {}^\omega \bm{J}^{\dot{s}}.
% \end{IEEEeqnarray}

